Distributed Mini-Batch SDCA

We present an improved analysis of mini-batched stochastic dual coordinate ascent for regularized empirical loss minimization (i.e. SVM and SVM-type objectives). Our analysis allows for flexible sampling schemes, including where data is distribute across machines, and combines a dependence on the smoothness of the loss and/or the data spread (measured through the spectral norm).

==> commands.tex <==
\usepackage{subfig}
\usepackage{tikz}
\usepackage{amsmath,hyperref}
\usepackage{pdflscape}
\usepackage{verbatim}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\newcommand{\theHalgorithm}{\arabic{algorithm}}
%\SetAlgorithmName{Algorithm Schema}{\autoref}{List of Algorithms}

\SetKwFor{ParallelForEach}{for each}{in parallel do}{endfor}

\newcommand{\TT}[0]{{\tau}}
\newcommand{\K}[0]{{\mathcal C}}

\newcommand{\Kidx}[0]{c}

\newcommand{\TP}[0]{{\mathcal P}}
\newcommand{\JJ}[0]{ D_i }
\newcommand{\GG}[0]{ D }


\DeclareMathOperator*{\proj}{proj}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Diag}{Diag}

\DeclareMathOperator*{\mysgn}{sgn}

\DeclareMathOperator*{\successor}{succ}
\DeclareMathOperator*{\predecessor}{pred}

\DeclareMathOperator*{\rroot}{root}
\DeclareMathOperator*{\rung}{rung}

\newcommand{\sets}[1]{\la #1 \ra}
\newcommand{\sgn}{sgn}


\newcommand{\note}[1]{{\color{red} #1}}
\newcommand{\error}[1]{{\tiny \color{red} #1}}

\newcommand{\vsubset}[2]{#1_{[#2]}}


\newcommand{\f}{f}
\newcommand{\YY}{\varphi}
 
\newcommand{\sK}{\mathcal{K}}
%\newcommand{\J}{J}
\newcommand{\sJ}{\mathcal{J}}


%\newcommand{\del}[1]{{\color{red} #1}}
%FIXME \usepackage{perpage}
\newcommand{\mycomment}[1]{\footnote{#1}}

\let\la=\langle
\let\ra=\rangle

\newcommand{\st}{\;:\;}
\newcommand{\ve}[2]{\langle #1 ,  #2 \rangle}

%\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{:=}

\newcommand{\ii}{{}^{(i)}}

\newcommand{\R}{\mathbf{R}}
\newcommand{\integers}{\mathbf{N}}
\newcommand{\Prob}{\mathbf{Prob}}
\newcommand{\E}{\mathbf{E}}


\newcommand{\pc}[2]{#1^{[#2]}}

\newcommand{\vc}[2]{#1^{\la #2 \ra}}
\newcommand{\bvc}[2]{#1^{(#2)}}
\newcommand{\vt}[2]{#1_{#2}}
\newcommand{\vct}[3]{#1^{#2}_{#3}}
\newcommand{\vPCc}[3]{#1^{\{#3\} : #2}}
\newcommand{\vPCt}[3]{#1^{#2}_{#3}}
\newcommand{\vPC}[2]{#1^{#2}}

\newcommand{\mrow}[2]{#1_{{#2}{:}}}
\newcommand{\mcol}[2]{#1_{{:}{#2}}}
\newcommand{\mel}[3]{#1_{{#2},{#3}}}

\newcommand{\Sj}[0]{{\hat Z}^{c}}


\newcommand{\G}[2]{#1^{(#2)}}
\newcommand{\dG}[2]{#1^{(#2)}}

\newcommand{\nc}[2]{{\color{red}\|#1\|_{(#2)}}}
\newcommand{\ncs}[2]{\|#1\|^2_{(#2)}}
\newcommand{\ncc}[2]{{\color{red}\|#1\|^*_{(#2)}}}
\newcommand{\ls}[1]{{\color{red} \mathcal S(#1)}}
\newcommand{\Rw}[2]{\mathcal R_{#1}(#2)}
\newcommand{\Rws}[2]{\mathcal R^2_{#1}(#2)}

\newcommand{\Rel}[2]{\mathcal {R}_{#1}^{#2}}


\newcommand{\nbp}[2]{\|#1\|_{(#2)}}   % norm block primal
\newcommand{\nbd}[2]{\|#1\|_{(#2)}^*} % norm block dual

\newcommand{\lf}{\mathcal L}
\newcommand{\U}{U}
\newcommand{\N}{N}

\newcommand{\mLi}{{\color{red}m^{(i)}}}
\newcommand{\gLi}{{\color{red}g^{(i)}}}
%\newcommand{\TLi}{{\color{red}T_L^{(i)}}}
\newcommand{\TLi}[1]{{\color{blue}T^{(#1)}}}
\newcommand{\TL}{{\color{blue}T}}

\newcommand{\support}{{\color{blue}support}}


\newcommand{\Lip}{L}
\newcommand{\ALip}{\tilde L}

\newcommand{\Rc}[1]{{\color{red}  \mathbf{RC}_{(#1)}}}
\newcommand{\NRCDM}{{\color{red}NRCDM}\  }
\newcommand{\nnz}[1]{\|#1\|_0}
% sets

\newtheorem{assumption}{Assumption}


\newcommand{\cBroadcast}{c_1}
\newcommand{\cNeighboursNo}{k_2}
\newcommand{\cNeighboursTime}{c_2}
\newcommand{\cPointToPoint}{c_3}
